Uncovering the Connections Between Adversarial Transferability and Knowledge Transferability

Knowledge transferability, or transfer learning, has been widely adopted to allow a pre-trained model in the source domain to be effectively adapted to downstream tasks in the target domain. It is thus important to explore and understand the factors affecting knowledge transferability. In this paper, as the first work, we analyze and demonstrate the connections between knowledge transferability and another important phenomenon--adversarial transferability, \emph{i.e.}, adversarial examples generated against one model can be transferred to attack other models. Our theoretical studies show that adversarial transferability indicates knowledge transferability and vice versa. Moreover, based on the theoretical insights, we propose two practical adversarial transferability metrics to characterize this process, serving as bidirectional indicators between adversarial and knowledge transferability. We conduct extensive experiments for different scenarios on diverse datasets, showing a positive correlation between adversarial transferability and knowledge transferability. Our findings will shed light on future research about effective knowledge transfer learning and adversarial transferability analyses.

==> [ICML21 Submission] Uncovering the Connections Between Adversarial Transferability and Knowledge Transferability/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm, amsthm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\rowsp}{rowsp}
\DeclareMathOperator{\colsp}{colsp}

\newtheorem{question}{Question}
\newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{conjecture}{Conjecture}
\newtheorem{problem}{Problem}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}

\numberwithin{theorem}{section}
\numberwithin{lemma}{section}
\numberwithin{proposition}{section}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
%\norm{ \biggl(\sum_{n=1}^N \mathbf{P}_{n}\biggr) }

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\supp}{\text{supp}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> [ICML21 Submission] Uncovering the Connections Between Adversarial Transferability and Knowledge Transferability/sections/abstract.tex <==
\begin{abstract}
% \textbf{Version 1:} Despite the immense success achieved by deep neural networks (DNNs), \emph{adversarial examples}, which are perturbed inputs that aim to mislead DNNs, have recently led to great concerns. On the other hand, adversarial examples exhibit interesting phenomena, such as \emph{adversarial transferability}. DNNs also exhibit knowledge transfer, which is critical to improving learning efficiency and learning in domains that lack high-quality training data. 
% %As adversarial transfer and knowledge transfer both connect source and target domains, it is especially interesting to see what are the relationships between the two behaviors. 
% %However, the connection between adversarial transferability and knowledge transferability is mostly unexplored. 
% %This manuscript proposes initial steps towards understanding the relationships between adversarial transfer and knowledge transfer.
% % To uncover the fundamental connections between these phenomena, we investigate and give an affirmative answer to the question: \emph{does adversarial transferability indicate knowledge transferability?} 
% %In this paper, we aim to turn the existence and pervasiveness of adversarial examples into an advantage. Given that adversarial transferability is easy to measure while it can be challenging to estimate the effectiveness of knowledge transfer, \emph{does adversarial transferability indicate knowledge transferability?} 
% We theoretically analyze the relations between adversarial transferability and knowledge transferability, and identify conditions when one corelates with the other. 
% %In particular, we show that composition with an affine function is sufficient to reduce the difference between the two models when they possess high adversarial transferability. 
% With the theoretical insights, we design a new metric complementary to adversarial transferability (to elaborate more). We provide empirical evaluation for different transfer learning scenarios on diverse datasets, showing a strong positive correlation between the adversarial transferability and knowledge transferability. Potential applications are discussed based on our theoretical and empirical findings. %thus illustrating that our theoretical insights are predictive of practice.

% Knowledge transferability, or transfer learning, has been widely adopted to allow a pre-trained model in the source domain to be effectively adapted to downstream tasks in the target domain.
% It is thus important to explore and understand the factors affecting knowledge transferability. 
% %There have been several studies to explore the factors that would affect such knowledge transferability, such as the accuracy and robustness of the pre-trained models. 
% In this paper, we analyze and demonstrate a previously under-explored connection between knowledge transferability and another important phenomenon--adversarial transferability, \emph{i.e.}, adversarial examples generated against one model can be transferred to attack other models. 
% %In this paper, as the first work, we aim to reveal the connection between knowledge transferability and adversarial transferability, which measures the model vulnerability when applying the perturbation generated against another model to it.
% Our theoretical study shows that adversarial transferability indicates knowledge transferability and vice versa. Moreover, based on the theoretical insights, we propose two practical adversarial transferability metrics to capture major information in the adversarial transfer process,  serving as bidirectional indicators of knowledge transferability. 
% %We theoretically analyze their relationship and identify a set of conditions for their positive correlations. In particular, we prove that xxx models with high adv, will have high knowledge transferability in terms of xxxxxx. We also prove that models with high knowledge transferability will more likely to be adversarial tranfer from one to another xxxxxx.
% We conduct extensive experiments for different transfer scenarios on diverse datasets, showing a positive correlation between adversarial transferability and knowledge transferability. Our findings provide inspirations and justifications for several interesting applications.

Knowledge transferability, or transfer learning, has been widely adopted to allow a pre-trained model in the source domain to be effectively adapted to downstream tasks in the target domain. It is thus important to explore and understand the factors affecting knowledge transferability. In this paper, as the first work, we analyze and demonstrate the connections between knowledge transferability and another important phenomenon--adversarial transferability, \emph{i.e.}, adversarial examples generated against one model can be transferred to attack other models. Our theoretical studies show that adversarial transferability indicates knowledge transferability, and vice versa. Moreover, based on the theoretical insights, we propose two practical adversarial transferability metrics to characterize this process,  serving as bidirectional indicators between adversarial and knowledge transferability. We conduct extensive experiments for different scenarios on diverse datasets, showing a positive correlation between adversarial transferability and knowledge transferability. Our findings will shed light on future research about effective knowledge transfer learning and adversarial transferability analyses. All code and data are available \href{https://github.com/AI-secure/Uncovering-the-Connections-BetweenAdversarial-Transferability-and-Knowledge-Transferability}{here}.



\end{abstract}


% \paragraph{Logic of the story}: 
% \begin{enumerate}
%     \item Knowledge transfer is important.
%     \item It is important to study factors that affect knowledge transfer (\textbf{Motivation 1})
%     \item We find that the process of adversarial transfer is a related to knowledge transfer (\textbf{Message 1}). \bo{emphasize this new and first to do so. adv transfer is important since there are many theoretical and empirical work on it}
%     \item We propose two practical adversarial transferability metrics to capture the information from the process of adversarial transfer. We propose to use the two proposed adversarial transferability as bidirectional indicators of KT. (\textbf{Message 2; Methods})
%     \item Our theory show that the process of adversarial transfer connects to the surrogate gradient knowledge transferability, and the gradient loss connects to the transfer loss. From the theoretical insights, the two metrics are justified. (\textbf{Theoretical justification for our messages and methods}) \bo{remember to use the adv transfer and knowledge transfer to represent these two, otherwise sometimes they could be confusing}
%     \item We further justify our claim and the two proposed adversarial transferabilities in experiments (\textbf{Experimental justification of our messages and methods}), which lead to potential applications.  (\textbf{Motivation 2})
% \end{enumerate}

==> [ICML21 Submission] Uncovering the Connections Between Adversarial Transferability and Knowledge Transferability/sections/adv_and_knowledge.tex <==
\section{Adversarial Transferability and Knowledge Transferability}\label{sec:preliminaries}
% \textbf{Contents:}
% \begin{enumerate}
%     \item Notations
%     \item Settings
%     \item definitions of adversarial attacks, and the two adversarial transferability metrics (The definition here is general, and can be applied to both theory and experiments).
%     \item Intuition about the two metrics, leading to theoretical analyses
% \end{enumerate}


This section introduces the preliminaries and the formal definitions of the knowledge and adversarial transferability, and formally defines our problem of interest. 
%Let us begin with the notations used throughout this paper, where some notations may offer a more fundamental perspective to understand the studied problem. 

\textbf{Notation.} Sets are denoted in blackboard bold, e.g., $\sR$, and the set of integers $\{1\dots n\}$ is denoted as $[n]$. Distributions are denoted in calligraphy, e.g., $\gD$, and the support of a distribution $\gD$ is denoted as $\supp(\gD)$. Vectors are denoted as bold lower case letters, e.g., $\vx \in \sR^n$, and matrices are denoted as bold uppercase letters, e.g., $\mW$. We denote the entry-wise product operator between vectors or matrices as $\odot$. The Moore–Penrose inverse of a matrix $\mW$ is denoted as $\mW^\dagger$.
We use $\|\cdot\|_2$ to denote Euclidean norm induced by Euclidean inner product $\langle \cdot, \cdot \rangle$.
The standard inner product of two matrices is defined as $\langle \mW, \mM \rangle=\tr(\mW^\top \mM)$, where $\tr(\cdot)$ is  the trace of a matrix. The Frobenius norm $\|\cdot\|_F$ is induced by the standard matrix inner product.
Moreover, in the (semi-)inner product space defined by a positive (semi-)definite matrix $\mS$, the (semi-)inner product of two vectors or matrices is defined by $\langle \vv_1, \vv_2 \rangle_\mS=\vv_1^\top \mS \vv_2$ or $\langle \mW, \mM \rangle_\mS=\tr(\mW^\top \mS \mM)$, respectively. Given a vector $\vv$, we define its normalization as $\widehat{\vv}=\vv / \|\vv\|_2$. When using a denominator $\|\cdot\|_*$ other than Euclidean norm, we denote the normalization as $\widehat{\vv}|_*$.
%Given a vector $\vv$, we define $(\vv)_*=\vv / \|\vv\|_*$ to be a unit-vector normalized under norm $\|\cdot\|_*$, \emph{e.g.}, $(\vv)_2$ denotes its unit-vector under Euclidean norm.

Given a (vector-valued) function $f$, we denote $f(\vx)$ as its evaluated value at $\vx$, and $f$ represents the function itself in the corresponding Hilbert space. 
Composition of functions is denoted as $g\circ f(\vx)=g(f(\vx))$. We use $\langle \cdot, \cdot \rangle_\gD$ to denote the inner product induced by distribution $\gD$ and inherited from Euclidean inner product, i.e., $\langle f_1, f_2 \rangle_\gD = \E_{\vx\sim \gD} \langle f_1(\vx), f_2(\vx)\rangle$.
Accordingly, we use $\|\cdot\|_{\gD}$ to denote the norm induced by the inner product $\langle \cdot, \cdot \rangle_\gD$, i.e., $\|f\|_{\gD}=\sqrt{\langle f, f \rangle_\gD}$. When the inherited inner product is defined by $\mS$, we denote $\langle f_1, f_2 \rangle_{\gD, \mS} = \E_{\vx\sim \gD} \langle f_1(\vx), f_2(\vx)\rangle_\mS$, and similarly for $\|f\|_{\gD, \mS}$. 


%For a matrix function $F:\supp(\gD)\to \sR^{d\times m}$, we define its $L^2(\gD)$-norm in accordance with matrix $2$-norm as $\|F\|_{\gD, 2}=\sqrt{\E_{\vx\sim \gD} \|F(\vx)\|_2^2}$. 
%For a general function $f:\sX\to\sY$, its $L^{\infty, 2}(\sX)$-norm is defined as $\|f\|_{\infty, 2}=\sup_{\vx \in \sX} \|f(\vx)\|_2 $.

%Equipped with the notation, we can formally defined the problem studied in this paper. 

\textbf{Knowledge Transferability}
%Let $\vx \in \sR^n$ and $y(\vx) \in \sR^d$. 
Given a pre-trained {\em source} model $f_S:\sR^n \to \sR^m$ and a {\em target} domain $\vx \in \sR^n$ with data distribution $\vx \sim \gD$ and {\em target} labels $y(\vx)\in \sR^d$, {\em knowledge transferability} is defined as the performance of fine-tuning $f_S$ on $\gD$ to predict $y$. Concretely, knowledge transferability can be represented as a loss $\Ls(\ \cdot \ , y, \gD)$ after fine-tuning by composing the fixed source model with a trainable function $g:\sR^m\to \sR^d$, typically from a small function class $g\in \sG$, \textit{i.e.},
\begin{align}
    \min_{g\in \sG} \quad  \Ls(g\circ f_S, y, \gD),  \label{def:knowledge-transf}
\end{align}
where the loss function $\Ls$ measures the error between $g\circ f_S$ and the ground truth $y$ under the {\em target} data distribution $\gD$. For example, for neural networks it is usual to stack on and fine-tune a linear layer; here $\sG$ is the affine function class. We will focus on the affine setting in this paper. 

%By instantiating the ground truth target $y$ by a target reference model $f_T:\sR^n\to \sR^d$, one can see something potentially interesting--how does their adversarial transferability connect to knowledge transferability? Hence, 
For our purposes, a more useful measure of transfer is to compare the quality of the fine-tuned model to a model trained directly on the target domain $f_T:\sR^n\to \sR^d$. Thus, we study the following surrogate of knowledge transferability, where the ground truth target is replaced by a reference target model $f_T$:
\begin{align}
    \min_{g\in \sG} \quad  \Ls(g\circ f_S, f_T, \gD).  \label{def:knowledge-transf-fT}
\end{align}
%Together with the source model and target model, let us introduce the process of adversarial transfer between them.

\begin{figure*}[t!]
    \centering
    \begin{minipage}{0.57\linewidth}
    \centering
        \includegraphics[width=\linewidth]{figures/figures-illustration-metrics.pdf}
        \small (a) 
    \end{minipage}
    \begin{minipage}{0.4\linewidth}
    \centering
        \includegraphics[width=\linewidth]{figures/figures-illustration-theory.pdf}
        \small (b) 
    \end{minipage}
    \caption{\small (a) An illustration of the two proposed adversarial transferability metrics $\alpha_1, \alpha_2$ under different adversarial transferability settings, \emph{i.e.}, $\alpha_1^{f_S\to f_T}, \alpha_1^{f_T\to f_S}, \alpha_2^{f_S\to f_T}$, and $\alpha_2^{f_T\to f_S}$. (b) An overview of the theoretical analysis framework, and its practical inspirations, where $\star, \diamond \in \{T, S\}$ and $\star \neq \diamond$. The three blue double-headed arrows are the bidirectional indication relationships proved in our theory section, and the dashed green arrow shows in practice how the two proposed adversarial transferability metrics are measured as representatives of the generalized adversarial transferability  based on our theory. 
    }
    \label{fig:theory-conclusion}
\end{figure*}

\textbf{Adversarial Attacks.}  
%The attack is generated so that a adversarial loss $\ell_{adv}(\cdot,\cdot)$ of the model output is maximized. 
For simplicity we consider untargeted attacks that seeks to maximize the deviation of model output
%after being attacked, 
as measured by a given adversarial loss function $\ell_{adv}(\cdot, \cdot)$. The targeted attack can be viewed as a special case. 
Without loss of generality, we assume the adversarial loss is \emph{non-negative}. 
Given a datapoint $\bm{x}$ and model $f$, an adversarial example of magnitude $\epsilon$ is denoted by $\bm{\delta}_{f,\epsilon}(\bm{x})$, computed as:
\begin{align}
    \bm{\delta}_{f,\epsilon}(\bm{x}) \ =\  \argmax_{\|\bm{\delta}\|\leq \epsilon} \   \ell_{adv}(f(\vx),f(\vx+\bm{\delta}) ). \label{def:adv-attack}
\end{align} 
We note that in theory $\bm{\delta}_{f,\epsilon}(\bm{x})$ may not be unique, and its generalized definition and its discussion are provided in our theoretical analysis (Section~\ref{sec:theory}). 
% For example, if we use squared loss with $l_2$-loss, we have
% \begin{align}
%     \bm{\delta}_{f,\epsilon}(\bm{x}) = \argmax_{\|\bm{\delta}\|\leq \epsilon} \|f(\vx)-f(\vx+\bm{\delta}) \|_2.
% \end{align}

\textbf{Adversarial Transferability.} The process of adversarial transfer involves applying the adversarial example generated against a model $f_1$ to another model $f_2$. Thus, adversarial transferability from $f_1$ to $f_2$ measures how well $\bm{\delta}_{f_1,\epsilon}$ attacks $f_2$. We propose two metrics, namely, $\alpha_1$ and $\alpha_2$ % defined in the following, 
that characterize adversarial transferability from complementary perspectives. To provide a visual overview of our definitions for the proposed adversarial transferability metrics, we present an illustration in Figure~\ref{fig:theory-conclusion} (a).
\begin{definition}[The First Adversarial Transferability]\label{def:alpha_1}
The first adversarial transferability from $f_1$ to $f_2$ at data sample $\vx\sim \gD$, is defined as
\begin{align}
    \alpha_1^{f_1\to f_2}(\vx) =\frac{\ell_{adv}(f_2(\vx),f_2(\vx+\bm{\delta}_{f_1, \epsilon}(\bm{x})) )}{\ell_{adv}(f_2(\vx),f_2(\vx+\bm{\delta}_{f_2, \epsilon}(\vx)) )} .
\end{align}
Taking the expectation, the first adversarial transferability is defined as
\begin{align}
    \alpha_1^{f_1\to f_2} =\E_{\vx\sim \gD}\left[ \alpha^{f_1\to f_2}(\vx)\right].
\end{align}
\end{definition}
Observe that the first adversarial transferability characterize how well the adversarial  attacks $\bm{\delta}_{f_1, \epsilon}$ generated against $f_1$ perform on $f_2$, compared to $f_2$'s whitebox adversarial attacks $\bm{\delta}_{f_2, \epsilon}$. Thus, high $\alpha_1$ indicates high adversarial transferability. Note that the two attacks use the same magnitude constraint $\epsilon$. 
%Formally, we consider transferred adversarial loss normalized by the its maximal adversarial loss given attack constraint $\epsilon$. 


Recall that $\ell_{adv}(f(\vx),f(\vx+\bm{\delta}) )$ measures the effect of the attack $\bm{\delta}$ on the model output $f(\vx)$. 
%(\emph{i.e.}, $f(\vx+\bm{\delta})$) deviates from  the original output $f(\vx)$, and we can see that 
$\alpha_1$ characterizes the relative magnitude of this deviation. However, this magnitude information is incomplete, as the direction of the deviation also encodes information about the adversarial transfer process. To this end, we propose the second adverserial metric, inspired by our theoretical analysis, which characterizes adversarial transferability from the directional perspective. 
\begin{definition}[The Second Adversarial Transferability]\label{def:alpha_2}
    The second adversarial transferability from $f_1$ to $f_2$, under data distribution $\vx\sim \gD$, is defined as
    \begin{align}
        \alpha_2^{f_1\to f_2}&=\|\E_{\vx\sim \gD}[ \widehat{\Delta_{f_1\to f_1}(\vx)} \widehat{\Delta_{f_1\to f_2}(\vx)}^\top ]\|_F,
    \end{align}
    where 
    \begin{align}
        \Delta_{f_1\to f_1}(\vx)&=f_1(\vx+\bm{\delta}_{f_1,\epsilon}(\vx))-f_1(\vx)\\
        \Delta_{f_1\to f_2}(\vx)&=f_2(\vx+\bm{\delta}_{f_1,\epsilon}(\vx))-f_2(\vx)
    \end{align}
    are deviations in model output given the adversarial attack $\bm{\delta}_{f_1,\epsilon}(\vx)$ generated against $f_1$, and $\widehat{\ \cdot\ }$ denotes the corresponding unit-length vector.
\end{definition}
To further clarify the second adversarial transferability metric, consider the following alternative form of $\alpha_2$. 
%in another form, such that the intuition behind $\alpha_2$ is clearer.
\begin{proposition} \label{prop:1} The $\alpha_2^{f_1\to f_2}$ can be reformulated as
\begin{align}
    (\alpha_2^{f_1\to f_2})^2   = \E_{\vx_1, \vx_2} \left[  \theta_{f_1\to f_1}(\vx_1, \vx_2)\theta_{f_1\to f_2}(\vx_1, \vx_2)\right],
\end{align}
where $\vx_1, \vx_2\overset{\text{i.i.d.}}{\sim}\gD$, and 
\begin{align}
    \theta_{f_1\to f_1}(\vx_1, \vx_2) &=\langle \widehat{\Delta_{f_1\to f_1}(\vx_1)}, \widehat{\Delta_{f_1\to f_1}(\vx_2)} \rangle \\
    \theta_{f_1\to f_2}(\vx_1, \vx_2) &=\langle \widehat{\Delta_{f_1\to f_2}(\vx_1)}, \widehat{\Delta_{f_1\to f_2}(\vx_2)} \rangle 
\end{align}
\end{proposition}
We can see that high $\alpha_2$ indicates that it is more likely for the two inner products (\emph{i.e.}, $\theta_{f_1\to f_1}$ and $\theta_{f_1\to f_2}$) to have the same sign. Given that the direction of $f_1$'s output deviation indicates its attack $\bm{\delta}_{f_1,\epsilon}$, and the direction of $f_2$'s output deviation indicates the transferred attack $\bm{\delta}_{f_1,\epsilon}$, high $\alpha_2$ implies that the two directions will rotate by a similar angle as the data changes.

% $\alpha_1$ and $\alpha_2$ represent complementary aspects of the adversarial transferability: 
% $\alpha_1$ can be understood as how often the adversarial attack transfers, while $\alpha_2$ encodes directional information of the output deviation caused by adversarial attacks. Recall that $\alpha_1, \alpha_2 \in [0,1]$ (higher values indicate better adversarial transferability). As we will show in our theoretical results reveal that high $\alpha_1$ alone is not enough, \textit{i.e.}, both the proposed metrics are necessary to characterize adversarial transferability and the relation between adversarial and knowledge transferabilities. 

% We provide a one-dimensional example showing that large $\alpha_1$ only is not enough to indicate high knowledge transferability. Suppose the ground truth target function $f_T(x) = x^2$, and the source function $f_S(x)=\texttt{sgn}(x)\cdot x^2$ where $\texttt{sgn}(\cdot)$ denotes the sign function. Let the adversarial loss be the deviation in function output, and the data distribution be the uniform distribution on $[-1, 1]$. As we can see, 
% %the direction that makes either $f_T$ or $f_S$ deviates the most is always the same, \textit{i.e.}, 
% {in this example even with $\alpha_1=1$ achieves its maximum and adversarial attacks always transfer. However, 
% there does not exist an affine function $g$ (\textit{i.e.}, fine-tuning) making $g\circ f_S$ close to $f_T$ on $[-1, 1]$}. Indeed, one can verify that $\alpha_2=0$ in this case, which contributes to the low knowledge transferability.
% However, if we move the data distribution to $[0, 2]$, we can have $\alpha_1=\alpha_2=1$ indicating high adversarial transferability, and indeed it achieves $f_S=f_T$ showing perfect knowledge transferability.

$\alpha_1$ and $\alpha_2$ represent complementary aspects of the adversarial transferability: 
$\alpha_1$ can be understood as how often the adversarial attack transfers, while $\alpha_2$ encodes directional information of the output deviation caused by adversarial attacks. An example is provided in the appendix section~\ref{sec:example-alpha} to illustrate the necessity of both the metrics in characterizing the relation between adversarial transferability and knowledge transferability.   To jointly take the two adversarial transferability metrics into consideration, we propose the following metric as the combined value of $\alpha_1$ and $\alpha_2$. 
\begin{align}
    &(\alpha_1 * \alpha_2)^{f_1\to f_2}=\\
    &\qquad \big\|\E_{\vx\sim \gD}[ \alpha_1^{f_1\to f_2}(\vx)\widehat{\Delta_{f_1\to f_1}(\vx)} \widehat{\Delta_{f_1\to f_2}(\vx)}^\top ]\big\|_F.
\end{align}

% \textbf{\textit{Maybe a figure here to illustrate $\alpha_1$ and $\alpha_2$. +1}} \bo{figure here}

%With the intuition, we can see that both $\alpha_1$ and $\alpha_2$ enjoy a nice property (Proposition~\ref{prop:2}).
We defer the justification for the combined adversarial transferability metric in the next section, and move on to state a useful proposition.
\begin{proposition}\label{prop:2}
The adversarial transferabililty metrics $\alpha_1^{f_1\to f_2}$, $\alpha_2^{f_1\to f_2}$ and $(\alpha_1 * \alpha_2)^{f_1\to f_2}$ are in $[0,1]$.
\end{proposition}
So far, we have defined knowledge transferability, and two adversarial trasferability metrics. We can now analyze their connections more precisely. 

\textbf{Problem of Interest.} Given a {\em source} model $f_S:\sR^n \to \sR^m$, the {\em target} data distribution $\vx\sim \gD$, the ground truth target $y:\sR^n\to \sR^d$, and a {\em target} reference model $f_T:\sR^n\to \sR^d$, we aim to study how the adversarial transferability between $f_S$ and $f_T$, characterized by the two proposed adversarial transferability metrics, connects to the knowledge transfer loss $\min_{g\in \sG}  \Ls(g\circ f_S, y, \gD)$ with affine functions $g\in \sG$ (\eqref{def:knowledge-transf}). 
% The adversarial transfer process is characterized by the two proposed adversarial transferability metrics $\alpha_1, \alpha_2$, and  with the surrogate knowledge transfer loss (\eqref{def:knowledge-transf-fT}). 

==> [ICML21 Submission] Uncovering the Connections Between Adversarial Transferability and Knowledge Transferability/sections/conclusion.tex <==
\section{Conclusion}
We theoretically analyze the relation between adversarial transferability and knowledge transferability. We provide empirical experimental justifications in pratical settings. Both our theoretical and empirical results show that adversarial transferability can indicate knowledge transferability and vice versa. We expect our work will inspire future work  on further exploring other factors that impact knowledge transferability and adversarial transferability.
%We hope our discovery can inspire and facilitate further investigations, such as model interpretability, fairness, robust and efficient transfer learning, and etc.

==> [ICML21 Submission] Uncovering the Connections Between Adversarial Transferability and Knowledge Transferability/sections/exp.tex <==
\section{Experimental Evaluation}\label{sec:exp}
%First show synthertic exp to connect theory to experiments, and then 
We present the real-data experiments based on both image and natural language datasets in this section, and discuss the  potential applications. 

% Inspired by our theoretical results, we conduct empirical experiments to showcase the practicality of the connection between adversarial transferability and knowledge transferability on real image and natural language datasets with common model architectures.

\textbf{Adversarial Transferability Indicating Knowledge Transferability. }
% When it comes to classification of images, there are many choices of neural network architectures, but there is little knowledge on how to choose the best one. 
In this experiment, we show how to use adversarial transferability to identify the optimal transfer learning candidates from a pool of models trained on the same source dataset.
We first train 5 different architectures (AlexNet, Fully connected network, LeNet,  ResNet18, ResNet50) on cifar10~\cite{krizhevsky2009learning}. Then we perform transfer learning to STL10~\cite{coates2011analysis} to obtain the knowledge transferability of each, measured by accuracy. At the same time, we also train one ResNet18 on STL10 as the target model, which has poor accuracy because of the lack of data. To measure the adversarial transferability, we generate adversarial examples with PGD~\cite{madry2017towards} on the target model and use the generated adversarial examples to attack each source model. The adversarial transferability is expressed in the form of $\alpha_1$ and $\alpha_2$. Our results in Table \ref{table:exp1} indicate that we can use adversarial tarnsferability to forecast knowledge transferability, where the only major computational overheads are training a naive model on the target domain and generating a few adversarial examples. In the end, We further evaluate the significance of our results by  Pearson score. More details about training and generation of adversarial examples can be found in the appendix~\ref{section:appendix_exp}.
\begin{table}[h]
    \centering
    \begin{small}
     \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{ccccc}
     \toprule
     \textbf{Model} &\textbf{Knowledge Trans.}&
     $\alpha_1$ &  
     $\alpha_2$ & 
     \textbf{$\alpha_1 * \alpha_2$}\\
     \midrule
    % Fully Connected & 28.30 & 0.279 & 0.117 & 0.0103\\
    % \hline
    % AlexNet & 45.65 & 0.614 & 0.208 & 0.0863\\
    % \hline
    % LeNet & 55.09 & 0.803 & 0.298 & 0.205\\
    % % \hline
    % % Transformer & 55.66 & 0.554 & 0.124 & 0.0444\\
    % \hline
    % ResNet18 & 76.60 & 1.000 & 0.405 & 0.410\\
    % \hline
    % ResNet50 & 77.92 & 0.962 & 0.392 & 0.368\\
    Fully Connected & 28.30 & 0.346 & 0.189 & 0.0258\\
    \hline
    LeNet & 45.65 & 0.324 & 0.215 & 0.0254\\
    \hline
    AlexNet  & 55.09 & 0.337 & 0.205 & 0.0268\\
    
    % \hline
    % Transformer & 55.66 & 0.554 & 0.124 & 0.0444\\
    \hline
    ResNet18 & 76.60 & 0.538 & 0.244 & 0.0707\\
    \hline
    ResNet50 & 77.92 & 0.614 & 0.234 & 0.0899\\
     \bottomrule
     \end{tabular}
     }
     \end{small}
     \vspace{-3mm}
    \caption{\small Knowledge transferability (Knowledge Trans.) among different model architectures. Our correlation  analysis shows Pearson score of -0.51 between the transfer loss and $\alpha_1$. Lower transfer loss corresponds to higher transfer accuracy. More details can be found in fig \ref{fig:exp1_pgd_img} in the Appendix~\ref{section:appendix_exp}} 
    \vspace{-3mm}
    \label{table:exp1}
\end{table}

To further validate our idea, we also conduct experiments on the NLP domain. We first finetune 5 different BERT classification models on different data domain (IMDB, Moview Review (MR), Yelp, AG, Fake). We refer the models trained on MR, Yelp, AG and Fake datasets as the source models, and take the model trained on IMDB datset as the target model. 
To measure the knowledge transferability, we fine-tune the source models with new linear layers on the target dataset for one epoch. We report the accuracy of the transferred models on the target test set as the metric to indicate the knowledge transferability. 
In terms of the adversarial transferability, we generate adversarial examples by the state-of-the-art whitebox attack algorithm T3 \citep{t3} against the target model and transfer the adversarial examples to source models to evaluate the adversarial transferability. Following our previous experiment, we also calculate $\alpha_1$ and $\alpha_2$. Experimental results are shown in Table \ref{table:nlp_exp1}. We observe that source models with larger adversarial transferability, measured by $\alpha_1$, $\alpha_2$ and $\alpha_1 * \alpha_2$, indeed tend to have larger knowledge transferability. 

% \begin{table}[h]
%     \centering
%     \begin{small}
%     \begin{tabular}{ccccc}
%      \toprule
%      \textbf{Model} &\textbf{Knowledge Trans.}&
%      $\alpha_1$ &  
%      $\alpha_2$ & 
%      $\alpha_1 * \alpha_2$\\
%      \midrule
%     MR & 89.34 & 0.975 & 0.00387 & 4.02e-3\\
%     \hline
%     Yelp & 88.81 & 0.610 & 0.00158 & 1.03e-3\\
%     \hline
%     AG  &  87.58 & 0.254 & 0.00076 & 1.15e-4 \\
%     \hline
%     Fake &  84.06 & 0.023 & 0.00102 & 6.18e-6\\
%      \bottomrule
%      \end{tabular}
%      \end{small}
%      \vspace{-3mm}
%     \caption{\small Knowledge transferability (Knowledge Trans.) from the Source Models (MR, Yelp, AG, Fake) to the Target Model (IMDB). Adversarial transferability is measured by using the adversarial examples generated against the Target Model (IMDB) to attack the Source Models and estimate $\alpha_1$ and $\alpha_2$.}
%     \vspace{-3mm}
%     \label{table:nlp_exp1}
% \end{table}

\begin{table}[h]
    \centering
    \begin{small}
    \begin{tabular}{ccccc}
     \toprule
     \textbf{Model} &\textbf{Knowledge Trans.}&
     $\alpha_1$ &  
     $\alpha_2$ & 
     $\alpha_1 * \alpha_2$\\
     \midrule
    MR & 89.34 & 0.743 & 0.00335 & 3.00e-3\\
    \hline
    Yelp & 88.81 & 0.562 & 0.00135 & 8.87e-4\\
    \hline
    AG  &  87.58 & 0.295 & 0.00021 & 8.56e-5 \\
    \hline
    Fake &  84.06 & 0.028 & 0.00032 & 5.58e-6\\
     \bottomrule
     \end{tabular}
     \end{small}
     \vspace{-3mm}
    \caption{\small Knowledge transferability (Knowledge Trans.) from the Source Models (MR, Yelp, AG, Fake) to the Target Model (IMDB). Adversarial transferability is measured by using the adversarial examples generated against the Target Model (IMDB) to attack the Source Models and estimate $\alpha_1$ and $\alpha_2$. The correlation analysis shows Pearson Score of $0.27$ between the transfer confidence and $\alpha_1$. Higher transfer confidence indicates higher knowledge transferability. More details can be found in Figure \ref{fig:exp1_nlp_img} in Appendix \S \ref{section:appendix_exp}.}
    \vspace{-3mm}
    \label{table:nlp_exp1}
\end{table}


\begin{table}[h]
    \centering
    \begin{small}
    \vspace{-3mm}
    \begin{tabular}{ccccc}
     \toprule
     \textbf{Similarity} &\textbf{Knowledge Trans.}&
     $\alpha_1$ &  
     $\alpha_2$ & 
     \textbf{$\alpha_1*\alpha_2$}\\
     \midrule
    0\% & 45.00 & 0.310 & 0.146 & 0.0169\\
    \hline
    25\% & 45.68 & 0.318 & 0.305 & 0.0383\\
    \hline
    50\% & 59.09 & 0.338 & 0.355 & 0.0436\\
    \hline
    75\% & 71.62 & 0.337 & 0.312 & 0.0402\\
    \hline
    100\% & 81.84 & 0.358 & 0.357 & 0.0489\\
     \bottomrule
     \end{tabular}
     \end{small}
     \vspace{-3mm}
    \caption{\small Knowledge transferability (Knowledge Trans.) of different source model. Similarity indicates how similar the source distributions are with the target distribution. Our correlation  analysis shows Pearson score of -0.06 between the transfer loss and $\alpha_1$. Lower transfer loss corresponds to higher knowledge transferability. More details can be found in fig \ref{fig:exp2_img} in the Appendix~\ref{section:appendix_exp}.}
    \vspace{-3mm}
    \label{table:exp2}
\end{table}

% \begin{table}[h]
%     \centering
%     \begin{small}
%     \begin{tabular}{ccccc}
%      \toprule
%      \textbf{Model} &\textbf{Knowledge Trans.}&
%      $\alpha_1$ &  
%      $\alpha_2$ & 
%      \textbf{$\alpha_1*\alpha_2$}\\
%      \midrule
%     MR & 89.34 & 0.997 & 0.00421 & 4.19e-3\\
%     \hline
%     Yelp & 88.81 & 0.694 & 0.00131 & 8.71e-4\\
%     \hline
%     AG  &  87.58 & 0.311 & 0.00020 & 9.35e-5\\
%     \hline
%     Fake &  84.06 & 0.205 & 0.00037 & 9.88e-5\\
%      \bottomrule
%      \end{tabular}
%      \end{small}
%      \vspace{-3mm}
%     \caption{\small Knowledge transferability (Knowledge Trans.) from the Source Models (MR, Yelp, AG, Fake) to the Target Model (IMDB). Adversarial transferability is measured by using the adversarial examples generated against the Source Models to attack the Target Models and estimate $\alpha_1$ and $\alpha_2$.}
%     \vspace{-3mm}
%     \label{table:nlp_exp2}
% \end{table}


\begin{table}[h]
    \centering
    \begin{small}
    \begin{tabular}{ccccc}
        % \boxin{
     \toprule
     \textbf{Model} &\textbf{Knowledge Trans.}&
     $\alpha_1$ &  
     $\alpha_2$ & 
     \textbf{$\alpha_1*\alpha_2$}\\
     \midrule
    MR & 89.34 & 0.584 & 0.00188 & 2.32e-3\\
    \hline
    Yelp & 88.81 & 0.648 & 0.00120 & 9.52e-4\\
    \hline
    AG  &  87.58 & 0.293 & 0.00016 &  4.35e-6 \\
    \hline
    Fake &  84.06 & 0.150 & 0.00073 & 3.55e-5\\
     \bottomrule
     \end{tabular}
     \end{small}
     \vspace{-3mm}
    \caption{\small Knowledge transferability (Knowledge Trans.) from the Source Models (MR, Yelp, AG, Fake) to the Target Model (IMDB). Adversarial transferability is measured by using the adversarial examples generated against the Source Models to attack the Target Models and estimate $\alpha_1$ and $\alpha_2$. The correlation analysis shows Pearson Score of $0.27$ between the transfer confidence and $\alpha_1$. Higher transfer confidence indicates higher knowledge transferability. More details can be found in Figure \ref{fig:exp2_nlp_img} in Appendix \S \ref{section:appendix_exp}. }
    \vspace{-3mm}
    \label{table:nlp_exp2}
\end{table}

\textbf{Knowledge Transferability Indicating Adversarial Transferability.}
In addition, we are interested in the impact of knowledge transferability on adversarial transferability. As predicted by our theory, the more knowledge transferable a source model is to the target domain, the more adversarial transferable it is.

We split cifar10 into 5 different subsets containing different percentages of animals and vehicles. We train a resNet18 on each of them as source models, which are later fine-tuned to obtained the knowledge transferability measured by accuracy. Then we train another resNet18 on a subset of stl10 that only contains vehicles. Different from the last experiment, we generate adversarial examples with PGD on each of the source models and transfer them to the target model. Table \ref{table:exp2} shows, the source model that transfers knowledge better generates more transferable adversarial examples. This implies we can use this relation to facilitate blackbox attack against a hidden target model, given some knowledge about the source and target domains. More details of training and generation of adversarial examples can be found in the appendix.

We evaluate the impact of knowledge transferability to adversarial transferability in the NLP domain as well. We mostly follow the setting describe in the previous section, where we have four source models and one target model, and the knowledge transferability from source models to the target model is measured by the accuracy of the transferred models on the target test set. The difference lies on the evaluation of the adversarial transferability, where we generate adversarial examples against the source models and evaluate their attack capability on the target model. As shown in Table \ref{table:nlp_exp2}, we note that when the source data domain is getting closer to the target data domain, the knowledge transferability grows, and the adversarial transferability also increases. More experimental details can be found in Appendix~\ref{section:appendix_exp}.


\textbf{Ablation Studies}
Following the settings in table \ref{table:exp1}, we conduct ablation studies (table \ref{tab:ablation}) on two additional attack methods, MI~\cite{tramer2017ensemble}, PGD-L2 and two additional $\epsilon$ with PGD, 2/225, 4/255, we discover that neither the attack method nor $\epsilon$ has significant impact on our conclusion.

\begin{table}[htbp!]
    \centering
    %  \resizebox{0.48\textwidth}{!}{
     
     \begin{minipage}[b]{\hsize}\centering
     \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{ccccc}
     \toprule
     \textbf{Model} &\textbf{Knowledge Trans.}&
     $\alpha_1$ &  
     $\alpha_2$ & 
     \textbf{$\alpha_1 * \alpha_2$}\\
     \midrule
     Fully Connected & 28.30 & 0.0985 & 0.0196 & 0.00027\\
    \hline
    LeNet & 45.65 & 0.2106 & 0.0259 & 0.00158\\
    \hline
    AlexNet  & 55.09 & 0.1196 & 0.0206 & 0.00037\\
    
    % \hline
    % Transformer & 55.66 & 0.554 & 0.124 & 0.0444\\
    \hline
    ResNet18 & 76.60 & 0.2739 & 0.0413 & 0.00405\\
    \hline
    ResNet50 & 77.92 & 0.1952 & 0.0320 & 0.00172\\
     \bottomrule
     \end{tabular}
     }
     %\vspace{-3mm}
     
     {\small $\epsilon=2/255$. Pearson score is -0.45.} 
     
     \end{minipage}
     
     \begin{minipage}[b]{\hsize}\centering
     \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{ccccc}
     \toprule
     \textbf{Model} &\textbf{Knowledge Trans.}&
     $\alpha_1$ &  
     $\alpha_2$ & 
     \textbf{$\alpha_1 * \alpha_2$}\\
     \midrule
     Fully Connected & 28.30 & 0.0974 & 0.0225 & 0.00029\\
    \hline
    LeNet & 45.65 & 0.2099 & 0.0309 & 0.00192\\
    \hline
    AlexNet  & 55.09 & 0.1283 & 0.0230 & 0.00048\\
    
    % \hline
    % Transformer & 55.66 & 0.554 & 0.124 & 0.0444\\
    \hline
    ResNet18 & 76.60 & 0.2853 & 0.0481 & 0.00496\\
    \hline
    ResNet50 & 77.92 & 0.2495 & 0.0414 & 0.00337\\
     \bottomrule
     \end{tabular}
    }
    
     {\small $\epsilon=4/255$. Pearson score is -0.49.} 
     \end{minipage}
     
     \begin{minipage}[b]{\hsize}\centering
     \resizebox{1.0\textwidth}{!}{
     \begin{tabular}{ccccc}
     \toprule
     \textbf{Model} &\textbf{Knowledge Trans.}&
     $\alpha_1$ &  
     $\alpha_2$ & 
     \textbf{$\alpha_1 * \alpha_2$}\\
     \midrule
     Fully Connected & 28.30 & 0.1678 & 0.0379 & 0.0013\\
    \hline
    LeNet & 45.65 & 0.0997 & 0.0503 & 0.0005\\
    \hline
    AlexNet  & 55.09 & 0.1229 & 0.0506 & 0.0009\\
    
    % \hline
    % Transformer & 55.66 & 0.554 & 0.124 & 0.0444\\
    \hline
    ResNet18 & 76.60 & 0.2731 & 0.0630 & 0.0052\\
    \hline
    ResNet50 & 77.92 & 0.3695 & 0.0550 & 0.0081\\
     \bottomrule
     \end{tabular}
     }
     
     {\small Attack with MI. Pearson score is -0.45.} 
    \vspace{1.5mm}
     \end{minipage}
     \begin{minipage}[b]{\hsize}\centering
     \resizebox{1.0\textwidth}{!}{
     \begin{tabular}{ccccc}
     \toprule
     \textbf{Model} &\textbf{Knowledge Trans.}&
     $\alpha_1$ &  
     $\alpha_2$ & 
     \textbf{$\alpha_1 * \alpha_2$}\\
     \midrule
     Fully Connected & 28.30 & 0.0809 & 0.0175 & 0.00018\\
    \hline
    LeNet & 45.65 & 0.2430 & 0.0190 & 0.00149\\
    \hline
    AlexNet  & 55.09 & 0.1101 & 0.0188 & 0.00031\\
    
    % \hline
    % Transformer & 55.66 & 0.554 & 0.124 & 0.0444\\
    \hline
    ResNet18 & 76.60 & 0.3619 & 0.0303 &  0.00464\\
    \hline
    ResNet50 & 77.92 & 0.2506 & 0.0237 & 0.00179\\
     \bottomrule
     \end{tabular}
     }
     
     %\vspace{-3mm}
     {\small $\ell_2$ attack with $\epsilon=1$. Pearson score is -0.40.} 
     \end{minipage}
    \label{tab:ablation}
     \vspace{-7mm}
    \caption{\small With varying attack methods and $\epsilon$, adversarial transferability is still correlated with knowledge transferability.} 
    %  }
     \vspace{-2mm}
\end{table}

==> [ICML21 Submission] Uncovering the Connections Between Adversarial Transferability and Knowledge Transferability/sections/intro.tex <==
\section{Introduction}
% \textbf{Contents}
% \begin{enumerate}
%     \item General introduction
%     \item motivation (why the studied problem is important)
%     \item related work
%     \item contributions
% \end{enumerate}
% Knowledge transferability and adversarial transferability are two fundamental properties emerging when a learned model transfers to other domains. 
Knowledge transfer is quickly becoming the standard approach for fast learning adaptation across domains. Also known as transfer learning or learning transfer, knowledge transfer has been a critical technology for enabling several real-world applications, including object detection~\cite{zhang2014facial}, image segmentation~\cite{kendall2018multi}, multi-lingual machine translation~\cite{dong2015multi}, and language understanding evaluation~\cite{wang2018glue}, among others.
% Long before it was formally defined, the computer vision community has exploited it to perform important visual manipulations~\citep{johnson2016perceptual}, such as style transfer and super-resolution, where pretrained VGG networks~\citep{simonyan2014very} are utilized to encode images into semantically meaningful features. 
For example, since the release of ImageNet~\citep{russakovsky2015imagenet}, pretrained ImageNet models (e.g., on TensorFlow Hub or PyTorch-Hub) have become the default option for the knowledge transfer source due to its broad coverage of visual concepts and compatibility with various visual tasks~\citep{huh2016makes}. Motivated by its importance, many studies have explored the factors associated with knowledge transferability. Most recently, \citet{salman2020adversarially} showed that more robust pretrained ImageNet models transfer better to downstream tasks, which reveals that \textit{adversarial training} helps to improve knowledge transferability.

In the meantime, \textit{adversarial transferability} has been extensively studied---a phenomenon that an adversarial instance generated against one model has high probability attack another one without additional modification~\citep{papernot2016transferability,goodfellow2014explaining,joon2017adversarial}. 
Hence, adversarial transferability is widely exploited in black-box attacks~\citep{ilyas2018black,liu2016delving, naseer2019cross}. 
A line of work has been conducted to bound the adversarial transferability based on model (gradient) similarity~\cite{tramer2017space}. 
Given that both \textit{adversarial transferability} and \textit{knowledge transferability} are impacted by certain model similarity and adversarial ML properties, in this work, we aim to conduct the \textit{first} study to analyze the connections between them and ask,

\begin{quoting}
\itshape
\vspace*{-0.2em}
 What is the fundamental connection between knowledge transferability and adversarial transferability? Can we measure one and indicate the other?
\vspace*{-0.1em}
\end{quoting}

% Theoretically, we propose two metrics to jointly represent the adversarial transferability, and prove that high adversarial transferability would indicate high knowledge transferability, through the analysis on the gradient matching distance and function matching distance. On the other hand, we also prove that high knowledge transferability indicates high adversarial transferability. We conduct synthetic data based experiments to verify our theoretical conclusions and key variables.

% Empirically, we conduct a range of experiments on both image and natural language datasets. We control the model architecture to measure the adversarial transferability and show its significant positive correlation with knowledge transferability. In the meantime, we control the data distribution distance to measure the knowledge transferability, and show its positive correlation with adversarial transferability. 

%As knowledge transfers, so do the adversarial examples. Knowledge transferability is a well studied phenomenon in which a learnt model from the source domain is leveraged in the target domain. The computer vision community has been utilizing this for important visual manipulations~\citep{johnson2016perceptual}, such as style transfer and super-resolution, where pretrained VGGs~\citep{simonyan2014very} are used to encode semantically meaningful features. In parallel, adversarial transferability is a phenomenon that adversarial examples not only attack the model on which they are generated, but also attack other models~\citep{goodfellow2014explaining,papernot2016transferability}. Hence, adversarial transferability is widely exploited in black-box attacks~\citep{ilyas2018black,liu2016delving}. In addition, many theoretical analyses are conducted to establish sufficient conditions of adversarial transferability~\citep{demontis2019adversarial,ma2018characterizing}. 
% Knowledge transferability and adversarial transferability both reveal parts of the nature of machine learning. As the two properties are surely important on their own, we find the relation between the two vastly interesting. For example, how do they fundamentally connect to each other? Is there any indicating relationships between the two? Can their connections inspire more effective transfer learning and new perspective for adversarial transferability? To answer these questions, we aim to uncover the connections between adversarial transferability and knowledge transferability. 

%In this paper, we begin by showing that adversarial transferability can indicate knowledge transferability and vice versa.
%, without considering if any model is robust against adversarial attacks. 
%Then motivated by our theoretical results, we design empirical experiments to show: this tie helps identify promising source models efficiently from a pool of candidates; it can also facilitate blackbox attacks against hidden models given vague knowledge about the target domain.

% To the best of our knowledge, this is the first work studying the fundamental relation between adversarial transferability and knowledge transferability both theoretically and empirically. This paper can be summarized as follows.
{\bf {Technical Contributions.}}
In this paper, we take the \textit{first} step
towards exploring the fundamental relation between adversarial transferability and knowledge transferability.
We make contributions on both theoretical
and empirical fronts.   
\vspace{-0.5cm}
\begin{itemize}[leftmargin=*,itemsep=-0.5mm]
        \vspace{-0.8em}
    \item We formally define the adversarial transferability for the \textit{first} time by considering all potential adversarial perturbation vectors. We then conduct thorough and novel theoretical analysis  to characterize the precise connection between adversarial transferability and knowledge transferability based on our definition. 
    
    \item In particular, we prove that high adversarial transferability will indicate high knowledge transferability, which can be represented as the distance in an inner product space defined by the Hessian of the adversarial loss.
    In the meantime, we prove that high knowledge transferability will indicate high adversarial transferability.
    
    \item Based on our theoretical insights, we propose two practical adversarial transferability metrics that quantitatively measure the adversarial transferability in practice. We then provide simulational results to verify how these metrics connect with the knowledge transferability in a bidirectional way.
    
    \item Extensive experiments justify our theoretical insights and the proposed adversarial transferability metrics, leading to our discussion on potential applications and future research.
\end{itemize}

\textbf{Related Work} There is a line of research studying different factors that affect knowledge transferability~\citep{yosinski2014transferable,long2015learning,wang2019characterizing,xu2019larger,shinya2019understanding}. Further, empirical observations show that the correlation between learning tasks~\citep{achille2019task2vec, zamir2018taskonomy}, the similarity of model architectures, and data distribution are all correlated with different knowledge transfer abilities. Interestingly, recent empirical evidence suggests that adversarially-trained models transfer  better than non-robust models \cite{salman2020adversarially, utrera2020adversarially}, suggesting a connection between the adversarial properties and knowledge transferability. On the other hand, several approaches have been proposed to boost the adversarial transferability~\citep{zhou2018transferable,demontis2019adversarial,dong2019evading,xie2019improving}. Beyond the above empirical studies, there are a few existing analyses of adversarial transferability, which explore different conditions that may enhance adversarial transferability~\citep{athalye2018obfuscated,tramer2017space,ma2018characterizing,demontis2019adversarial}. 
In this work, we aim to bridge the connection between adversarial and knowledge transferability, both of which reveal interesting properties of ML model similarities from different perspectives.

% Recent interest in the relation between knowledege transferability and adversarial robustness has led to some fruitful discoveries \cite{joon2017adversarial, utrera2020adversarially}. Empirically, it is shown that adversarially robust models transfer knowledge better than non-robust models. In stark contrast, scarce attention has been paid to another orthogonal but equally important topic, the relation between knowledge transferability and adversarial transferability. 
% % However, a more effective indicator of knowledge transferability is required to quantitatively understand its effectiveness or feasibility in a computational realistic way even before one conducts the expensive training and fine-tuning process. 

% Adversarial Transferability has been observed by several works~\citep{papernot2016transferability,goodfellow2014explaining,joon2017adversarial}. Since the early work, a lot of studies have been conducted, aiming to further understand the phenomenon and design more transferable adversarial attacks. Regardless of the threat model, a lot of attack methods have been proposed to boost adversarial transferability~\citep{zhou2018transferable,demontis2019adversarial,dong2019evading,xie2019improving}. 
% \cite{naseer2019cross} propose to produce adversarial examples that transfer cross-domain via a generative adversarial network. 
% In addition to the efficacy, efficiency~\citep{ilyas2018black} and practicality~\citep{papernot2017practical} are also optimized.   
% Beyond the above empirical studies, there is some work dedicated to analyzing this phenomenon, showing different conditions that may enhance adversarial transferability~\citep{athalye2018obfuscated,tramer2017space,ma2018characterizing,demontis2019adversarial}.



% \textbf{Knowledge transferability} has been widely applied in scenarios where the available data for certain domain is limited, and has achieved great success~\citep{van2014transfer,wurm2019semantic,wang2017self,kim2017end,maqueda2018event,devlin2018bert}. 
% Several studies have been conducted to understand the factors that affect knowledge transferability~\citep{yosinski2014transferable,long2015learning,wang2019characterizing,xu2019larger,shinya2019understanding}. Empirical observations show that the correlation between learning tasks~\citep{achille2019task2vec, zamir2018taskonomy}, the similarity of model architectures, and data distribution are all correlated with different knowledge transfer effects. 
% % However, a more effective indicator of knowledge transferability is required to quantitatively understand its effectiveness or feasibility in a computational realistic way even before one conducts the expensive training and fine-tuning process. 

% \textbf{Adversarial Transferability} has been observed by several works~\citep{papernot2016transferability,goodfellow2014explaining,joon2017adversarial}. Since the early work, a lot of studies have been conducted, aiming to further understand the phenomenon and design more transferable adversarial attacks. Regardless of the threat model, a lot of attack methods have been proposed to boost adversarial transferability~\citep{zhou2018transferable,demontis2019adversarial,dong2019evading,xie2019improving}. 
% \cite{naseer2019cross} propose to produce adversarial examples that transfer cross-domain via a generative adversarial network. 
% In addition to the efficacy, efficiency~\citep{ilyas2018black} and practicality~\citep{papernot2017practical} are also optimized.   
% Beyond the above empirical studies, there is some work dedicated to analyzing this phenomenon, showing different conditions that may enhance adversarial transferability~\citep{athalye2018obfuscated,tramer2017space,ma2018characterizing,demontis2019adversarial}.
% Building upon these %great understandings and
% observations, it is clear that there exist certain connections between adversarial transferability and other knowledge transfer scenarios, and here we aim to provide the first theoretic justification to verify it and design systematic empirical studies to measure such correlation.

==> [ICML21 Submission] Uncovering the Connections Between Adversarial Transferability and Knowledge Transferability/sections/synthetic-exp.tex <==
\section{Synthetic Experiments}\label{sec:synthetic-exp}
% Synthetic experiments using 1-hidden layer NN on Gaussian mixture data. Verify some properties that are intractable to verify on large-scale experiment. Bridge the gap between theory and practice.

% \textbf{Contents}:
% \begin{enumerate}
%     \item compute the gradient matching distance exactly, comparing it with the function matching distance and the transfer loss. 
%     \item show factors other than the two metrics.
%     \item compare results with varying model width. 
% \end{enumerate}
The synthetic experiment aims to bridge the gap between theory and practice by verifying some of the theoretical insights that may be difficult to compute for large-scale experiments.  Specifically, the synthetic experiment aims to verify: first, how influential are the two proposed adversarial transferability metrics $\alpha_1, \alpha_2$ comparing to the other factors in the generalized adversarial attacks (\eqref{def:generalized-attack}); Second, how does the gradient matching distance track the knowledge transfer loss. The dataset ($N=5000$) is generated by a Gaussian mixture of $10$ Gaussians. The ground truth target is set to be the sum of $100$ radial basis functions. The dimension of $\vx$ is $50$, and the dimension of the target is $10$. Details of the datasets are defer to appendix section~\ref{sec:appendix-synthetic-exp}.

\textbf{Models} Both the source model $f_S$ and target model $f_T$ are one-hidden-layer neural networks with sigmoid activation.

% \textbf{Dataset}
% Denote a radial basis function as $\phi_i(\vx) = e^{-\|\vx-\bm{\mu}_i\|_2^2/(2\sigma_i)^2}$, and we set the target ground truth to be the sum of $M=100$ basis functions as $y=\sum_{i=1}^M \phi_i$, where each entry of the parameters are sampled once from $U(-0.5, 0.5)$. We set the dimension of $\vx$ to be $50$, and the dimension of the target to be $10$. We generate $N=5000$ samples of $\vx$ from a Gaussian mixture formed by $10$ Gaussians with different centers but the same covariance matrix $\mathbf{\Sigma}=\mI$. The centers are sampled randomly from $U(-0.5, 0.5)^n$. We use the ground truth target function $y(\cdot)$ to derive the corresponding data $\vy$ for each $\vx$. That is, we want our neural networks to approximate $y(\cdot)$ on the Gaussian mixture. 

\textbf{Methods} First, sample $D=\{(\vx_i, \vy_i)\}_{i=1}^N$ from the distribution, where $\vx$ is $50$-dimensional, $\vy$ is $10$-dimensional. 
Then we train a target model $f_T$ on $D$.
To derive the source models, we first train a target model on $D$ with width $m = 100$. Denoting the weights of a target model as $\mW$, we randomly sample a direction $\mV$ where each entry of $\mV$ is sampled from $U(-0.5, 0.5)$, and choose a scale $t\in [0, 1]$. Subsequently, we perturb the model weights of the clean source model as $\mW’ := \mW + t\mV$, and define the source model $f_S$ to be a one-hidden-layer neural network with weights $\mW’$. 
Then, we compute each of the quantities we care about, including $\alpha_1$, $\alpha_2$ from both $f_S\to f_T$ and $f_T\to f_S$, the gradient matching distance (\eqref{def:gradient-matching-dist}), and the actual knowledge transfer distance (\eqref{def:know-transfer-dist}). We use the standard $\ell_2$ loss as the adversarial loss function.

\textbf{Results} 
We present two sets of experiment in Figure~\ref{fig:exp-synthetic}. The indication relations between adversarial transferability and knowledge transferability can be observed. Moreover: 1. the metrics $\alpha_1, \alpha_2$ are more meaningful if using the regular attacks $\bm{\delta}_{f_\star}^{(1)}$; 2. the gradient matching distance tracks the actual knowledge transferability loss; 3. the directions of $f_T\to f_S$ and $f_S \to f_T$ are similar.
\begin{figure}[h!]\centering
    \begin{minipage}{0.4\linewidth}\centering
        \includegraphics[width=\linewidth]{figures/synthetic-fig-1.png}
        {\small (a) $\bm{\delta}_{f_\star}^{(1)}$}
    \end{minipage}
    \begin{minipage}{0.4\linewidth}\centering
        \includegraphics[width=\linewidth]{figures/synthetic-fig-2.png}
        {\small (b) $\bm{\delta}_{f_\star}^{(2)}$}
    \end{minipage}
    \vspace{-3mm}
    \caption{ \small As defined in \eqref{def:generalized-attack}, (a) corresponds to the regular adversarial attacks, while (b) the secondary adversarial attack. That is, (b) represents the other information in the adversarial transferring process compared with the first.  The x-axis shows the scale of perturbation $t\in [0,1]$ that controls how much the source model deviates from the target model. There are in total 6 quantities reported. Specifically, $\alpha_1^{f_T\to f_S}$ is \textbf{black solid}; $\alpha_1^{f_S\to f_T}$ is \textbf{black dotted};  $\alpha_2^{f_T\to f_S}$ is \textcolor{green}{\textbf{green solid}}; $\alpha_2^{f_S\to f_T}$ is \textcolor{green}{\textbf{green dotted}}; the gradient matching loss is \textcolor{red}{\textbf{red solid}}; and the knowledge transferability distance is  \textcolor{blue}{\textbf{blue solid}}.
    }
    \vspace{-5mm}
    \label{fig:exp-synthetic}
\end{figure}

%The correlations between adversarial transferabilities ($\tau_1, \tau_2, \alpha$) and the knowledge transferability (knowledge transfer loss) are observed. 
%The upper bound for the difference of gradients (Theorem~\ref{theorem:2}) basically tracks its true value. Although the absolute value of the upper bound on the transferred loss (Theorem~\ref{theorem:loss}) can be big compared to the true transferred loss, their trends are similar. We note the big difference in absolute value is due to the use of $\beta$-smoothness, which considers the worst case scenario. It is also observed that $\tau_1$ tracks the normalized adversarial cross loss $\alpha$, as Proposition~\ref{prop:2} suggests.

==> [ICML21 Submission] Uncovering the Connections Between Adversarial Transferability and Knowledge Transferability/sections/theory.tex <==
\section{Theoretical Analysis}\label{sec:theory}
In this section, we present the theoretical analysis on how the adversarial transferability and the knowledge transfer process are tied together. 
%Note that in the previous section, we use $f_1, f_2$ to represent two arbitrary functions. 
To simplify the discussion, as the objects studied in this section are specifically focused on the source domain $S$ and the target domain $T$, we can use $\star$ or $\diamond$ as a placeholder for either $S$ or $T$ throughout this section. 
%That being said, $\star, \diamond\in \{S, T\}$ to be specified. 
%After introducing the settings studied in this section, the analysis is divided into three parts. 

\textbf{Theoretical Analysis Overview.} 
%We begin by introducing the setting considered in this section. 
%As is standard, we consider adversarial transfer in the regime where the magnitude of adversarial pertubations is small. 
In subsection~\ref{subsec:theory-1}, we define the two \textit{generalized adversarial transferabilities}, (\textit{i.e.}, $\mA_1$, $\mA_2$), and present Theorem~\ref{theorem-1} showing that $\mA_1$, $\mA_2$ together determine a gradient matching distance $\min_{g\in \sG}\|\nabla f_\star- \nabla g\circ f_\diamond\|$, between the Jacobian matrices of the source and target models in an inner product space defined by the Hessian of the adversarial loss function. In the same subsection, we also show that $\alpha_1$ and $\alpha_2$ represent the most influential factors in $\mA_1$ and $\mA_2$, respectively. Next, we explore the connection to knowledge transferability in subsection~\ref{subsec:theory-2} via Theorem~\ref{theorem-2} which shows the gradient matching distance approximates the function matching distance, \emph{i.e.}, $\min_{g\in \sG}\|f_\star- g\circ f_\diamond\|$, with a distribution shift up to a Wasserstein distance. Finally, in subsection~\ref{subsec:theory-conclusion} we complete the analysis by outlining the connection between the function matching distance and the knowledge transfer loss. A visual overview is shown in Figure~\ref{fig:theory-conclusion} (b).
%, leading to the conclusion of the theoretical analysis.
%After the pure theoretical analysis, in subsection~\ref{subsec:synthetic-exp} we present a set of synthetic experiments that verify the theoretical insights from our results, leading to the empirical experiments in section~\ref{sec:exp}.

\textbf{Setting.} As adversarial perturbations are constrained in a small $\epsilon$-ball, it is reasonable to approximate the deviation of model outputs by its first-order Taylor approximation. Specifically, in this section we consider the Euclidean $\epsilon$-ball. Therefore, the output deviation of a function $f$ at $\vx$ given a small perturbation $\|\bm{\delta}_\epsilon\|_2\leq \epsilon$ can be approximated by
\begin{align}
  f(\vx + \bm{\delta}_\epsilon) - f(\vx) \approx \nabla f(\vx)^\top\bm{\delta}_\epsilon,
\end{align}
where $\nabla f(\vx)$ is the Jacobian matrix of $f$ at $\vx$.

We consider a convex and twice-differentiable adversarial loss function $\ell^\star_{adv}(\cdot)$ that measures the deviation of model output $f_\star(\vx + \bm{\delta}_\epsilon) - f_\star(\vx)$, with minimum $\ell^\star_{adv}(\bm{0})=0$, for $\star\in\{S,T\}$. We note that we should treat the adversarial loss on $f_S$ and $f_T$ differently, as they may have different output dimensions.  Accordingly, the adversarial attack (\eqref{def:adv-attack}) can be written as
\begin{align}\label{def:adv-attack-grad}
    \bm{\delta}_{f_\star,\epsilon}(\vx)\ =\ \argmax_{\|\bm{\delta}\|_2\leq \epsilon}\  \ell^\star_{adv}(\nabla f_\star(\vx)^\top\bm{\delta}).
\end{align}
% where $\star\in \{S,T\}$.
Another justification of the small-$\epsilon$ approximation follows the literature; since the ideal attack defined in \eqref{def:adv-attack} is often intractable to compute, much of the literature uses the proposed formulation (\ref{def:adv-attack-grad}) in practice, \emph{e.g.}, see \cite{miyato2018virtual}, with experimental results suggesting similar behaviour as the standard definition.

% For the knowledge transfer loss, to simplify the presentation, we consider the classic $\ell_2$-distance, which can be easily translated to a wide range of loss functions, \emph{e.g.,}, Lipschitz functions, mean squared error, and any loss function that can be represented 


%Let us defer the definition of the gradient matching distance for now, and 
\textbf{The Small-$\epsilon$ Regime.} 
%In the studied regime, where we omit the higher-order terms of $\epsilon$, the adversarial transfer process appears in an interesting form.
%
Recall that the adversarial loss $\ell^\star_{adv}(\cdot)$ studied in this section is convex, twice-differentiable, and achieves its minimum at $\bm{0}$, thus in the small $\epsilon$ regime:
\begin{align}
    \ell^\star_{adv}(\nabla f_\star(\vx)^\top\bm{\delta}_\epsilon) &= \left(\bm{\delta}_\epsilon^\top \nabla f_\star(\vx)\mH_\star \nabla f_\star(\vx)^\top\bm{\delta}_\epsilon \right)^{1/2}\\
    &= \|\nabla f_\star(\vx)^\top\bm{\delta}_\epsilon\|_{\mH_\star},
\end{align}
which is the norm of $f_\star$'s output deviation in the inner product space defined by the Hessian $\mH_\star$ of the squared adversarial loss $(\ell_{adv}^\star)^2$.

Accordingly, the adversarial attacks (\ref{def:adv-attack-grad}) can be written as
\begin{align}\label{def:adv-attack-norm}
     \bm{\delta}_{f_\star,\epsilon}(\vx)\ =\ \argmax_{\|\bm{\delta}\|_2\leq \epsilon}\  \|\nabla f_\star(\vx)^\top\bm{\delta}\|_{\mH_\star}, 
\end{align} 
and we can measure the output deviation of $f_\diamond$'s caused by $f_\star$'s adversarial attack $ \bm{\delta}_{f_\star, \epsilon}(\vx)$, denoted as:
\begin{align}\label{def:deviation-small}
    \Delta_{f_\star\to f_\diamond, \epsilon}(\vx)=\nabla f_\diamond(\vx)^\top \bm{\delta}_{f_\star, \epsilon}(\vx).
\end{align}
% where $\star, \diamond\in \{S, T\}$.
%Consequently, we can re-write $\alpha_1$ in Definition~\ref{def:alpha_1} in a concrete form. 
Note that in the small-$\epsilon$ regime, the actual value of $\epsilon$ becomes trivial (\emph{e.g., $\alpha_1$}), consequently we will omit the $\epsilon$ for notational ease:
\begin{align}
    \alpha_1^{f_\star\to f_\diamond}(\vx) &=\frac{\|\Delta_{f_\star\to f_\diamond}(\vx)\|_{\mH_\diamond}}{\|\nabla f_\diamond(\vx)\|_{\mH_\diamond}} .
\end{align}
Similarly, $\alpha_2$ can be computed using (\ref{def:deviation-small}) in Definition~\ref{def:alpha_2}, \emph{i.e.},
\begin{align}
    \alpha_2^{f_\star\to f_\diamond}&=\|\E_{\vx\sim \gD}[ \widehat{\Delta_{f_\star\to f_\star}(\vx)} \widehat{\Delta_{f_\star\to f_\diamond}(\vx)}^\top ]\|_F.
\end{align}
With these insights, next we will derive our first theorem.

\subsection{Adversarial Transfer Indicates the Gradient Matching Distance, and Vice Versa}\label{subsec:theory-1}
% \textbf{Contents}: 
% \begin{enumerate}
%     \item show that the gradient matching distance can be characterised by the two aspects of adversarial transfer. (Theorem 1)
%     \item Discuss and justify the two proposed metrics
% \end{enumerate}
% introduce the settings studied specific to theoretical study. Present the results and their interpretations, showing that the generalized (multi-value) alpha and beta (former name: gamma) precisely decide the surrogate knowledge transfer loss. From the theoretical results, we can see the (single-value) alpha and beta (former name: gamma) are the most influential ones in their generalized version.  %From the theoretical insights, define the new metric complementary to the adv transferability.
% In the regime of small $\epsilon$, an interesting result can be derived.
We present an interesting finding in this subsection, \emph{i.e.}, the generalized adversarial transferabilities $\mA_1, \mA_2$ have a direct connection to the gradient matching distance between the source model $f_S:\sR^n\to \sR^m$ and target model $f_T:\sR^n\to\sR^d$. The gradient matching distance is defined as the smallest distance an affine transformation can achieve between their Jacobians $\nabla f_T: \sR^n \to \sR^{n\times d}$ and $\nabla f_S :\sR^n\to \sR^{n\times m}$ in the inner product space defined by $\mH_\star$ and data sample distribution $\vx \sim \gD$, as shown below.
\begin{align}\label{def:gradient-matching-dist}
    \min_{g\in \sG} \quad \|\nabla f_\star^\top -  \nabla(g\circ f_\diamond)^\top\|_{\gD, \mH_\star},
\end{align}
where $g\in \sG$ are affine transformations. Note that $g: \sR^m \to \sR^d$ if $(\star, \diamond)=(T,S)$, and $g: \sR^d \to \sR^m$ if $(\star, \diamond)=(S,T)$. 
We defer the analysis of how the gradient matching distance approximates the knowledge transfer loss, and focus on its connection to adversarial transfer. 

\textbf{A Full Picture of Adversarial Transferability.} A key observation is that the adversarial attack (\eqref{def:adv-attack-norm}) is the singular vector corresponding to the largest singular value of the Jacobian $\nabla f_\star(\vx)$ in the $\mH_\star$ inner product space. Thus, information regarding other singular values that are not revealed by the adversarial attack. Therefore, we can consider other singular values, corresponding to smaller signals than the one revealed by adversarial attacks, to complete the analysis.
We denote $\bm{\sigma}_{f_\star, \mH_\star}(\vx)\in \sR^n$ as the descending (in absolute value) singular values of the Jacobian $\nabla f_\star(\vx)^\top \in \sR^{\cdot \times n}$ in the $\mH_\star$ inner product space. In other words, we denote $\bm{\sigma}_{f_\star, \mH_\star}(\vx)\in \sR^n$ as the square root of the descending eigenvalues of $\nabla f_\star(\vx) \mH_\star \nabla f_\star(\vx)^\top$, \textit{i.e.},
\begin{align} \label{def:sigma}
    \bm{\sigma}_{f_\star, \mH_\star}(\vx)=
        [\sigma_{f_\star}^{(1)}(\vx),
        \dots ,
        \sigma_{f_\star}^{(n)}(\vx)]^\top.
\end{align}
Note that the number of non-zero singular values may be less than $n$, in which case we fill the rest with zeros such that vector is $n$-dimensional. 
% Note that we use $\sigma_f(\vx)$ to denote the largest singular value of the Jacobian $\nabla f(\vx)$. To generalize the notion, we use vectors (bold symbol) 

Since the adversarial attack $\bm{\delta}_{f_\star,\epsilon}(\vx)$ corresponds to the largest singular value $\sigma_{f_\star}(\vx)^{(1)}$, we can also generalize the adversarial attack by including all the singular vectors. \emph{i.e.},
\begin{align}\label{def:generalized-attack}
     \bm{\delta}_{f_\star}^{(i)}(\vx) \quad \text{ corresponds to }\quad \sigma_{f_\star}^{(i)}(\vx),\quad \forall i\in [n].
\end{align}
Loosely speaking, one could think $\bm{\delta}_{f_\star}^{(i)}(\vx)$ as the adversarial attack of $f_\star(\vx)$ in the subspace orthogonal to all the previous attacks, \emph{i.e.}, $\bm{\delta}_{f_\star}^{(j)}(\vx)$ for $\forall j\in[i-1]$.

Accordingly, for $\forall i\in[i]$ we denote the output deviation as
\begin{align}\label{def:generalied-Delta}
    \Delta^{(i)}_{f_\star\to f_\diamond}(\vx)=\nabla f_\diamond(\vx)^\top \bm{\delta}_{f_\star}^{(i)}(\vx).
\end{align} 
As a consequence, we \textit{generalize the first adversarial transferability} to be a $n$-dimensional vector $\bm{A}_1^{\star, \diamond}(\vx)$ including the adversarial losses of all of the generalized adversarial attacks, where the $i^{th}$ element in the vector is
\begin{align}
    \bm{A}_1^{\star, \diamond}(\vx)^{(i)}=\frac{\|\Delta_{f_\star\to f_\diamond}^{(i)}(\vx)\|_{\mH_\diamond}}{\|\nabla f_\diamond (\vx)\|_{\mH_\diamond}}. \label{def:alpha-1-generalized}
\end{align}
Note that the first entry of $\bm{A}_1^{\star, \diamond}(\vx)$ is the original adversarial transferability, \emph{i.e.},  ${\mA}_1^{\star, \diamond}(\vx)^{(1)}$ is the same as the ${\alpha}_1^{f_\star\to f_\diamond}(\vx)$ in Definition~\ref{def:alpha_1}.

With the above generalization that captures the full picture of the adversarial transfer process, we able to derive the following theorem.
\begin{theorem}\label{theorem-1}
Given the target and source models $f_\star, f_\diamond$, where $(\star, \diamond)\in\{(S, T), (T,S)\}$, the gradient matching distance (\eqref{def:gradient-matching-dist}) can be written as
    \begin{align}
        & \min_{g\in \sG} \quad \|\nabla f_\star^\top -  \nabla(g\circ f_\diamond)^\top\|_{\gD, \mH_\star}= \label{eq:theorem-1}\\
        & \sqrt{1-\frac{\E[\vv^{\star,\diamond}_{}(\vx_1)^\top {\mA}_2^{\star,\diamond}({\vx_1, \vx_2}) \vv^{\star,\diamond}_{}(\vx_2)]  }{\|\nabla f_\star^\top\|_{\gD, \mH_\star}^2\cdot \|\mJ^\dagger\|^{-1}_{\mH_\diamond}} }\|\nabla f_\star^\top\|_{\gD, \mH_\star},
    \end{align}
    where the expectation is taken over $\vx_1, \vx_2 \overset{\text{i.i.d.}}{\sim} \gD$, and
    \begin{align}
        \vv^{\star,\diamond}_{}(\vx)&=\sigma^{(1)}_{f_\diamond, \mH_\diamond}(\vx)\bm{\sigma}_{f_\star, \mH_\star}(\vx) \odot \mA_1^{\star, \diamond}(\vx)\\
        \mJ&=\E_{\vx\sim\gD} [\nabla f_\diamond(\vx)^\top \nabla f_\diamond(\vx)].
    \end{align}
    Moreover, ${\mA}_2^{\star,\diamond}({\vx_1, \vx_2})$ is a matrix, and its element in the $i^{th}$ row and $j^{th}$ column is 
    \begin{align}
        {\mA}_2^{\star,\diamond}(\vx_1, \vx_2&)^{(i, j)}=\langle \widehat{ \Delta^{(i)}_{f_\star\to f_\star}(\vx_1)}  \big |_{\mH_\star}, \widehat{ \Delta^{(j)}_{f_\star\to f_\star}(\vx_2)}\big |_{\mH_\star} \rangle\\
        &\cdot \langle \widehat{ \Delta^{(i)}_{f_\star\to f_\diamond}(\vx_1)}\big |_{\mH_\diamond}, \widehat{ \Delta^{(j)}_{f_\star\to f_\diamond}(\vx_2)}\big |_{\mH_\diamond} \rangle_{\widehat{ \mJ^\dagger}|_{\mH_\diamond}} .
    \end{align}
\end{theorem}
Recall the alternative representation of the second adversarial transferability $\alpha_2$, and we can immediately observe that $\alpha_2$ is determined by $\mA_2$. Therefore, both $\alpha_1$ and $\alpha_2$ appear in this relation. Let us interpret the theorem, and justify the two proposed adversarial transferability metrics. 

\textbf{Interpretation of Theorem~\ref{theorem-1}.} First, we consider components that are not directly related to the adversarial transfer in the RHS of (\ref{eq:theorem-1}). The $\|\nabla f_\star^\top\|_{\gD, \mH_\star}$ outside represents the overall magnitude of the loss. In the fraction, the $\|\nabla f_\star^\top\|_{\gD, \mH_\star}$ in the denominator normalizes the $\bm{\sigma}_{f_\star}$ in the numerator. Similarly, though more complicated, the $\|\mJ^\dagger\|^{-1}_2$ in the denominator corresponds to the $\sigma_{f_\diamond}^{(1)}$ in the numerator. We note that these are properties of $f_\star, f_\diamond$. 

Next, observe that the components directly related to the adversarial transfer process are the \textit{generalized adversarial transferability} $\mA_1$ and $\mA_2$. Let us neglect the superscript $^{(i)}$ or $^{(j)}$ for now, so we can see that their interpretations are the same as we introduced for $\alpha_1$ and $\alpha_2$ in section~\ref{sec:preliminaries}. That is, $\mA_1$ captures the magnitude of the deviation in model outputs caused by adversarial attacks, while $\mA_2$ captures the direction of the deviation. A minor difference between $\alpha_2$ and $\mA_2$ is that the second inner product in the elements of $\mA_2$ is defined by a positive semi-definite matrix $\widehat{\mJ^\dagger}$. For practical implementation, we choose to neglect this term, and use the standard Euclidean inner product in $\alpha_2$, which can be understood as a stretched version of the $\widehat{\mJ^\dagger}$ inner product space. 

Moreover, as the singular vector $\bm{\sigma}_{f_\star}$ has descending entries, we can see that in the vector $\mA_1$ and the matrix $\mA_2$, the elements with superscript $^{(1)}$ have the most influence in the relations. In other words, the two proposed adversarial transferability metrics, $\alpha_1$ and $\alpha_2$, are the most influential factors in \eqref{eq:theorem-1}.  We can also see that the combined metric $(\alpha_1*\alpha_2)$ also stems from here by only considering the components with the first superscript.

To interpret the relation between the gradient matching distance and the adversarial transferabilities, we introduce the following proposition. This shows that, in general, $\mA_1$ and $\mA_2$ with their elements closer to $1$ can serve as a bidirectional indicator of a smaller gradient matching distance. 
\begin{proposition}\label{prop:3}
    In Theorem~\ref{theorem-1}, 
    \begin{align}
        0 \leq\frac{\E[\vv^{\star,\diamond}_{}(\vx_1)^\top \mA_2^{\star,\diamond}({\vx_1, \vx_2}) \vv^{\star,\diamond}_{}(\vx_2)]  }{\|\nabla f_\star^\top\|_{\gD, \mH_\star}^2\cdot \|\mJ^\dagger\|^{-1}_{\mH_\diamond}} \leq 1.
    \end{align}
\end{proposition}
In conclusion, Theorem~\ref{theorem-1} reveals a bidirectional relation between the adversarial transfer process and the gradient matching distance, where the adversarial transfer process can be encoded by the generalized adversarial transferabilities, \emph{i.e.}, $\mA_1$ and $\mA_2$. Moreover, $\alpha_1$ and $\alpha_2$ play the most influential role in their generalization, \textit{i.e.,} $\mA_1$ and $\mA_2$. 


\subsection{The Gradient Matching Distance indicates the Function Matching Distance, and Vice Versa}\label{subsec:theory-2}
%\bo{don't use single word transfer or transfer loss in this paper since transfer can mean two types. how about we call knowledge transfer, but use gradient matching distance to measure it. otherwise it could be confusing from the title}

%\bo{3.1 and 3.2 may just use: A as an indicator of B; vice versa. Currently they read no difference?}
% \begin{enumerate}
%     \item show that the function matching distance (surrogate transfer loss) can be upper bounded and lower bounded by some terms about the gradient matching distance, up to a distribution shift with bounded Wasserstein distance. (Theorem 2)
%     \item show that the transfer loss can be upper and lower bounder by the  function matching distance (surrogate transfer loss). (Proposition)
%     \item bring all the pieces together and make the conclusion of theoretical analysis.
% \end{enumerate}
To bridge the gradient matching distance to the knowledge transfer loss, an immediate step is to connect the gradient distance to the function distance which directly serves as a surrogate knowledge transfer loss as defined in (\eqref{def:knowledge-transf-fT}).
%That is being said, 
Specifically, in this subsection, we present a connection between the function matching distance, \emph{i.e.},
\begin{align}\label{def:function-matching-dist}
    \min_{g\in \sG} \  \| f_\star - g\circ f_\diamond\|_{\gD, \mH_\star},
\end{align}
and the gradient matching distance, \emph{i.e.},
\begin{align}\label{def:gradient-matching-dist-new}
   \min_{g\in \sG} \ \|\nabla f_\star^\top - \nabla (g\circ f_\diamond)^\top\|_{\gD, \mH_\star},
\end{align}
where $g\in \sG$ are affine transformations. 
%Note that $g: \sR^m \to \sR^d$ if $(\star, \diamond)=(T,S)$, and $g: \sR^d \to \sR^m$ if $(\star, \diamond)=(S,T)$. 

For intuition, consider a point $\vx_0$ in the input space $\sR^{n}$, a path $\gamma_\vx:[0,1]\to \sR^{n}$ such that $\gamma_\vx(0) = \vx_0$ and $\gamma_\vx(1)=\vx$. Then, denoting $\gamma$ as the function of $\vx$, we can write the difference between the two functions as
\begin{align}
    f_\star - {g}\circ f_\diamond = &\int_0^1 (\nabla f_\star(\gamma(t)) - \nabla (g \circ f_\diamond(\gamma(t))))^\top \dot{\gamma}(t) \diff t\\
    &+( f_\star(\vx_0)- g\circ f_\diamond(\vx_0))  .
\end{align}
Noting that the function difference is a path integral of the gradient difference, we should expect a distribution shift when characterizing their connection, \emph{i.e.}, the integral path affects the original data distribution $\gD$. Accordingly, as the integral path may leave the support of $\gD$, it is necessary to assume the smoothness of the function, as shown below. 

Denoting the optimal $g\in \sG$ in (\ref{def:function-matching-dist}) as $\Tilde{g}$, and one of the optimal $g\in \sG$ in (\ref{def:gradient-matching-dist-new}) as $\Tilde{g}'$, we define
\begin{align}
    h_{\star, \diamond} :=f_\star - \Tilde{g}\circ f_\diamond \quad \text{and} \quad h_{\star, \diamond}' :=f_\star - \Tilde{g}'\circ f_\diamond, \label{def:h}
\end{align}
and we can see that the gradient matching distance and the function matching distance can be written as
\begin{align}
    (\ref{def:function-matching-dist}) = \|h_{\star, \diamond}\|_{\gD, \mH_\star}  \quad \text{and} \quad (\ref{def:gradient-matching-dist-new}) = \|\nabla {h'_{\star, \diamond}}^\top\|_{\gD, \mH_\star}.
\end{align}
\begin{assumption}[$\beta$-smoothness]\label{assum:smooth}
   We assume $h_{\star, \diamond}$ and $h'_{\star, \diamond}$ are both $\beta$-smooth, \emph{i.e.},
    \begin{align}
        \|\nabla h_{\star, \diamond}^\top (\vx_1)-\nabla h_{\star, \diamond}^\top (\vx_2)\|_{\mH_\star} \leq \|\vx_1-\vx_2\|_{2},
    \end{align}
    and similarly for $h'_{\star, \diamond}$.
\end{assumption}
With this assumption, we can prove that the gradient matching distance and the function matching distance can bound each other. 
\begin{theorem}\label{theorem-2}
With the notation defined in \eqref{def:h}, assume the $\beta$-smoothness assumption holds. Given a data distribution $\gD$ and $\tau>0$, there exist distributions $\gD_1, \gD_2$ such that the type-1 Wasserstein distance $W_1(\gD, \gD_1)\leq \tau$ and $W_1(\gD, \gD_2)\leq \tau$ satisfying
    \begin{align}
        {\tfrac{1}{2B^2 }}\|h_{\star, \diamond}\|^2_{\gD, \mH_\star} &\leq \|\nabla h_{\star, \diamond}'^\top\|^2_{\gD_1, \mH_\star}+\beta^2(B-\tau)_+^2\\
        \tfrac{1}{3n}\|\nabla h_{\star, \diamond}'^\top\|^2_{\gD, \mH_\star}&\leq \tfrac{2}{\tau^2} \|h_{\star, \diamond}\|^2_{\gD_2, \mH_\star}+\beta^2\tau^2,
    \end{align}
    where $n$ is the dimension of $\vx\sim\gD$, and $B=\inf_{\vx_0\in \sR^n} \sup_{\vx \in \supp(\gD)} \|\vx-\vx_0\|_2$ is the radius of $\supp(\gD)$.
\end{theorem}
We note that the above theorem compromises some tightness in exchange for a cleaner presentation without losing its core message, which is discussed in the proof of the theorem. 

\textbf{Interpretation of Theorem~\ref{theorem-2}.} The theorem shows that under the smoothness assumption, the gradient matching distance indicates the function matching distance, and vice versa, with a distribution shift bounded in Wasserstein distance. As the distribution shift is in general necessary, we conjecture that using different data distributions for adversarial transfer and knowledge transfer can also be applicable.

\subsection{The Function Matching Distance Indicates Knowledge Transferability, and Vice Versa} \label{subsec:theory-conclusion}
To complete the story, it remains to connect the function matching distance to knowledge transferability. As the adversarial transfer is symmetric (\emph{i.e.}, either from $f_S\to f_T$ or $f_T\to f_S$), we are able to use the placeholders $\star, \diamond \in \{S, T\}$ all the way through. However, as the knowledge transfer is asymmetric (\emph{i.e.}, $f_S\to y$ to the target ground truth), we need to instantiate the direction of adversarial transfer to further our discussion. 

\textbf{Adversarial Transfer from $f_T\to f_S$.} As we can see from the $\mA_1^{\star, \diamond}$ in Theorem~\ref{theorem-1}, this direction corresponds to $(\star, \diamond) = (T, S)$. Accordingly, the function matching distance  (\eqref{def:function-matching-dist}) becomes
\begin{align}
        \min_{g\in \sG} \  \| f_T - g\circ f_S\|_{\gD, \mH_T}.\label{eq:function-distance-S-T}
\end{align}
We can see that \eqref{eq:function-distance-S-T} directly translates to the surrogate knowledge transfer loss that uses the ``pseudo ground truth'' from the target reference model $f_T$.

In other words, the function matching distance serves as an approximation of the knowledge transfer loss defined as their distance in the inner product space of $\mH_T$, \emph{i.e.},
%, \emph{i.e.}, the Hessian of the adversarial loss function $\ell_{dv}$.
\begin{align}
    \min_{g\in \sG} \ \| y - g\circ f_S\|_{\gD, \mH_T}. \label{def:know-transfer-dist}
\end{align}
The accuracy of the approximation depends on the performance of $f_T$, as shown in the following theorem.
\begin{theorem}\label{prop:4} The surrogate transfer loss (\ref{eq:function-distance-S-T}) and the true transfer loss (\ref{def:know-transfer-dist}) are close, with an error of  $\| f_T - y\|_{\gD, \mH_T}$.
\begin{align}
       -\| f_T - y\|_{\gD, \mH_T} \leq (\ref{def:know-transfer-dist})-(\ref{eq:function-distance-S-T}) \leq  \| f_T - y\|_{\gD, \mH_T}
\end{align}
\end{theorem}

\textbf{Adversarial Transfer from $f_S\to f_T$.} This direction corresponds to $(\star, \diamond) = (S, T)$. Accordingly, the function matching distance  (\eqref{def:function-matching-dist}) becomes
\begin{align}
    \min_{g\in \sG} \  \| f_S - g\circ f_T\|_{\gD, \mH_S}. \label{eq:function-distance-T-S}
\end{align}
Since the affine transformation $g$ acts on the target reference model, it can not be directly viewed as a surrogate transfer loss. However, interesting interpretations can be found in this  direction, depending on the output dimension of $f_S:\sR^n \to \sR^m$ and $f_T:\sR^n \to \sR^d$. 
%Denote the optimal solution for \eqref{eq:function-distance-T-S} as $\Tilde{g}$, and 

% Suppose $g:\sR^d \to \sR^m$ is full rank, and loosely speaking we can derive the following intuitions. If $d<m$, then $g$ is injective and there exists $g':\sR^m \to \sR^d$ such that $g'\cdot g$ is identity. That is, if $g$ can map $f_T$ to closely track $f_S$, then reversely $g'$ can map $f_S$ to $f_T$, showing that (\ref{eq:function-distance-T-S}) upper bounds (\ref{eq:function-distance-S-T}) in some sense. On the contrary, if $d>m$ then $g$ is surjective, and (\ref{eq:function-distance-S-T}) upper bounds (\ref{eq:function-distance-T-S}) in some sense. It is when $m=d$ that (\ref{eq:function-distance-S-T}) and (\ref{eq:function-distance-T-S}) coincide. 

That is, when the direction of adversarial transfer is from $f_S\to f_T$, the indicating relation between it and knowledge transferability would possibly be unidirectional, depending on the dimensions. More discussion is included in the appendix section~\ref{sec:adv-direction} due to space limitation. 


% \textbf{Conclusion of the Theoretical Analysis.} Combin
